PolyFit: Polynomial-based Indexing Approach for Fast Approximate Range Aggregate Queries

Range aggregate queries find frequent application in data analytics. In some use cases, approximate results are preferred over accurate results if they can be computed rapidly and satisfy approximation guarantees. Inspired by a recent indexing approach, we provide means of representing a discrete point data set by continuous functions that can then serve as compact index structures. More specifically, we develop a polynomial-based indexing approach, called PolyFit, for processing approximate range aggregate queries. PolyFit is capable of supporting multiple types of range aggregate queries, including COUNT, SUM, MIN and MAX aggregates, with guaranteed absolute and relative error bounds. Experiment results show that PolyFit is faster and more accurate and compact than existing learned index structures.

==> EDBT2021/Experiment0_SCALE/COUNT1D/plotcommand <==
set term wxt size 450,350 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.0 dataset records (million)}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xtics ("0" 0, "20" 20, "40" 40, "60" 60, "80" 80, "100" 100)
set ytics ("0" 0, "200" 200, "400" 400, "600" 600)

set xrange[0:*]
set yrange[0:600]
#set logscale x
#set logscale y

set lmargin 10.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment0_SCALE\\COUNT1D\\S2"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment0_SCALE\\COUNT1D\\FitingTreeNew"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment0_SCALE\\COUNT1D\\RMI"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment0_SCALE\\COUNT1D\\Polyfit"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment0_SCALE\\COUNT1D\\PGM"

set key spacing 2
set key top left
#set key top center horizontal

set title "{/*2.0 Q_{abs}}" offset 0,-0.5

# with RMI
# plot file3 using 1:2 title "{/*2.0 RMI}" ls 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*2.0 FITing-Tree}" ls 3 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*2.0 PGM}" ls 8 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*2.0 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints

# without RMI
plot file2 using 1:2 title "{/*2.0 FITing-Tree}" ls 3 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*2.0 PGM}" ls 8 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*2.0 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment0_SCALE/COUNT2D/plotcommand <==
set term wxt size 450,350 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.0 dataset records (million)}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xtics ("0" 0, "20" 20, "40" 40, "60" 60, "80" 80, "100" 100)

set xrange[0:*]
#set logscale x
set logscale y

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment0_SCALE\\COUNT2D\\Polyfit"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment0_SCALE\\COUNT2D\\aRtree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment0_SCALE\\COUNT2D\\MRTree"

set key spacing 2
set key center right
#set key top center horizontal

set title "{/*2.0 Q_{abs}}" offset 0,-0.5

plot file2 using 1:2 title "{/*2.0 aR-tree}" ls 8 lw 3 ps 2 with lines, file3 using 1:2 title "{/*2.0 MRTree}" lc 7 pt 11 lw 3 ps 2 with linespoints, file1 using 1:2 title "{/*2.0 PolyFit-3}" lc 9 pt 13 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment1_Time_Eabs/COUNT1D/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"

set xtics ("0" 0, "250" 250, "500" 500, "750" 750, "1000" 1000)
set xrange [0:*]

#set logscale x
set logscale y

set lmargin 14.5
set rmargin 10.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT1D\\S2"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT1D\\FitingTree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT1D\\RMI"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT1D\\Polyfit"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT1D\\PGM"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT1D\\RadixSpline"
file7 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT1D\\MRTree"

set key spacing 1.4
#set key bottom left
set key outside
set key top right

set size square 1,1

# COMPARE WITHOUT SAMPLING
plot file3 using 1:2 title "{/*1.5 RMI}" ls 4 lw 3 ps 2 with linespoints, file7 using 1:2 title "{/*1.5 MRTree}" lc 9 pt 14 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 FITing-Tree}" ls 3 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*1.5 PGM}" ls 8 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file6 using 1:2 title "{/*1.5 RadixSpline}" ls 10 lw 3 ps 2 with linespoints

# COMPARE WITH S2 ONLY
#plot file1 using 1:2 title "{/*1.5 S2}" ls 2 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment1_Time_Eabs/COUNT1D/plotcommand_2 <==
set term wxt size 600,450 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.5 absolute error threshold}" offset 0,-0.5
set ylabel "{/*2.5 query response time (ns)}" offset -1.8,0
set ylabel rotate by 90
set tics font "Helvetica,18"

set xtics ("0" 0, "500" 500, "1000" 1000, "1500" 1500, "2000" 2000)
set xrange [0:*]

#set logscale x
set logscale y

set lmargin 14.5
set rmargin 10.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT1D\\S2"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT1D\\FitingTree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT1D\\RMI"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT1D\\Polyfit"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT1D\\PGM"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT1D\\RadixSpline"
file7 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT1D\\MRTree"
file8 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT1D\\aRtree"

#set key off
set key spacing 1.4
set key bottom left horizontal
#set size ratio 0.8

set title "{/*2.5 Q_{abs}}" offset 0,-0.5

# COMPARE WITHOUT SAMPLING
plot file8 using 1:2 title "{/*2.0 aR-tree}" ls 8 lw 3 ps 2 with lines, file3 using 1:2 title "{/*2.0 RMI}" ls 4 lw 3 ps 2 with linespoints, file7 using 1:2 title "{/*2.0 MRTree}" lc 7 pt 11 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*2.0 FITing-Tree}" ls 3 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*2.0 PGM}" ls 8 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*2.0 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints


# COMPARE WITH S2 ONLY
#plot file1 using 1:2 title "{/*1.5 S2}" ls 2 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment1_Time_Eabs/COUNT2D/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"

set xtics ("0" 0, "250" 250, "500" 500, "750" 750, "1000" 1000)
set xrange [0:*]

#set logscale x
set logscale y

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT2D\\S2"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT2D\\aRtree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT2D\\Polyfit"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT2D\\MRTree"
#file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT2D\\VerdictDB"


set key spacing 1.4
set key outside
set key top right

set size square 1,1

# without S2
plot file4 using 1:2 title "{/*1.5 MRTree}" lc 9 pt 14 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 aR-tree}" ls 8 lw 3 ps 2 with lines, file3 using 1:2 title "{/*1.5 PolyFit-3}" lc 9 pt 13 lw 3 ps 2 with linespoints

# S2
#plot file1 using 1:2 title "{/*1.5 S2}" ls 2 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints


#"{/*1.5 MRTree}" lc 9 pt 14 lw 3 ps 2 with linespoints
#"{/*1.5 Polyfit-1}" ls 3 lw 3 ps 2 with linespoints
#"{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints
#"{/*1.5 PolyFit-3}" lc 9 pt 13 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment1_Time_Eabs/COUNT2D/plotcommand_2 <==
set term wxt size 600,450 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.5 absolute error threshold}" offset 0,-0.5
set ylabel "{/*2.5 query response time (ns)}" offset -2.5,0
set ylabel rotate by 90
set tics font "Helvetica,18"

set xtics ("0" 0, "1000" 1000, "2000" 2000, "3000" 3000, "4000" 4000)
set xrange [0:*]

#set logscale x
set logscale y

set lmargin 16.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT2D\\S2"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT2D\\aRtree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT2D\\Polyfit"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT2D\\MRTree"
#file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\COUNT2D\\VerdictDB"


set key spacing 2
set key at 1650, 50000
#set size ratio 0.8

set title "{/*2.5 Q_{abs}}" offset 0,-0.5

# without S2
plot file2 using 1:2 title "{/*2.0 aR-tree}" ls 8 lw 3 ps 2 with lines, file4 using 1:2 title "{/*2.0 MRTree}" lc 7 pt 11 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*2.0 PolyFit-3}" lc 9 pt 13 lw 3 ps 2 with linespoints

# S2
#plot file1 using 1:2 title "{/*1.5 S2}" ls 2 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints


#"{/*1.5 MRTree}" lc 9 pt 14 lw 3 ps 2 with linespoints
#"{/*1.5 Polyfit-1}" ls 3 lw 3 ps 2 with linespoints
#"{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints
#"{/*1.5 PolyFit-3}" lc 9 pt 13 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment1_Time_Eabs/MAX/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"

set xtics ("0" 0, "250" 250, "500" 500, "750" 750, "1000" 1000)
set xrange [0:*]
#set logscale x
set logscale y

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\MAX\\aMaxTree"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\MAX\\MRTree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\MAX\\Polyfit"

set key spacing 1.4
set key center right
#set key bottom left

set size square 1,1

plot file1 using 1:2 title "{/*1.5 aR-tree}" ls 8 lw 3 ps 2 with lines, file2 using 1:2 title "{/*1.5 MRTree}" lc 9 pt 14 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-1}" ls 6 lw 3 ps 2 pt 9 with linespoints

==> EDBT2021/Experiment1_Time_Eabs/MAX/plotcommand_2 <==
set term wxt size 450,350 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"

set xtics ("0" 0, "250" 250, "500" 500, "750" 750, "1000" 1000)
set xrange [0:*]
#set logscale x
set logscale y

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\MAX\\aMaxTree"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\MAX\\MRTree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment1_Time_Eabs\\MAX\\Polyfit"

set key spacing 1.4
set key at 980,1200
#set key center right
#set key bottom left

#set size square 1,1

set title "{/*2.0 Q_{abs}}" offset 0,-0.5

plot file1 using 1:2 title "{/*1.5 aR-tree}" ls 8 lw 3 ps 2 with lines, file2 using 1:2 title "{/*1.5 MRTree}" lc 7 pt 11 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-3}" ls 9 lw 3 ps 2 pt 13 with linespoints

==> EDBT2021/Experiment2_Time_Erel/COUNT1D/command <==
set style fill pattern 1 border
set xlabel "{/*2.0 relative error threshold}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
#set xtics ("0.005" 0.005, "0.01" 0.01, "0.05" 0.05, "0.1" 0.1, "0.2" 0.2)

set logscale x
set logscale y

set lmargin 14.5
set rmargin 10.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\S2"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\FitingTree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\RMI"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\Polyfit"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\PGM"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\RadixSpline"


set key spacing 1.4
#set key bottom left
#set key center right
set key outside
set key top right

set size square 1,1


# COMPARE WITHOUT SAMPLING
plot file3 using 1:2 title "{/*1.5 RMI}" ls 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 FITing-Tree}" ls 3 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*1.5 PGM}" ls 8 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file6 using 1:2 title "{/*1.5 RadixSpline}" ls 10 lc 10 pt 6 lw 3 ps 2 with linespoints


# COMPARE WITH S2 ONLY
#plot file1 using 1:2 title "{/*1.5 S2}" ls 2 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints


==> EDBT2021/Experiment2_Time_Erel/COUNT1D/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 relative error threshold}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
#set xtics ("0.005" 0.005, "0.01" 0.01, "0.05" 0.05, "0.1" 0.1, "0.2" 0.2)

set logscale x
set logscale y

set lmargin 14.5
set rmargin 10.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\S2"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\FitingTree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\RMI"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\Polyfit"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\PGM"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\RadixSpline"


set key spacing 1.4
#set key bottom left
#set key center right
set key outside
set key top right

set size square 1,1


# COMPARE WITHOUT SAMPLING
plot file3 using 1:2 title "{/*1.5 RMI}" ls 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 FITing-Tree}" ls 3 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*1.5 PGM}" ls 8 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file6 using 1:2 title "{/*1.5 RadixSpline}" ls 10 lw 3 ps 2 with linespoints


# COMPARE WITH S2 ONLY
#plot file1 using 1:2 title "{/*1.5 S2}" ls 2 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints


==> EDBT2021/Experiment2_Time_Erel/COUNT1D/plotcommand_2 <==
set term wxt size 600,450 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.5 relative error threshold}" offset 0,-0.5
set ylabel "{/*2.5 query response time (ns)}" offset -1.8,0
set ylabel rotate by 90
set tics font "Helvetica,18"
#set xtics ("0.005" 0.005, "0.01" 0.01, "0.05" 0.05, "0.1" 0.1, "0.2" 0.2)

set logscale x
set logscale y

set lmargin 14.5
set rmargin 10.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\S2"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\FitingTree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\RMI"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\Polyfit"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\PGM"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\RadixSpline"
file7 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\MRTree"
file8 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT1D\\aRtree"

#set key off
set key spacing 1.4
set key bottom left horizontal
#set size ratio 0.8

set title "{/*2.5 Q_{rel}}" offset 0,-0.5

# COMPARE WITHOUT SAMPLING
plot file8 using 1:2 title "{/*2.0 aR-tree}" ls 8 lw 3 ps 2 with lines, file3 using 1:2 title "{/*2.0 RMI}" ls 4 lw 3 ps 2 with linespoints, file7 using 1:2 title "{/*2.0 MRTree}" lc 7 pt 11 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*2.0 FITing-Tree}" ls 3 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*2.0 PGM}" ls 8 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*2.0 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints


# COMPARE WITH S2 ONLY
#plot file1 using 1:2 title "{/*1.5 S2}" ls 2 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints


==> EDBT2021/Experiment2_Time_Erel/COUNT2D/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 relative error threshold}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"

set logscale x
set logscale y

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT2D\\S2"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT2D\\aRtree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT2D\\Polyfit"


set key spacing 1.4
#set key top right
#set key center right
set key outside
set key top right

set size square 1,1

#plot file1 using 1:2 title "{/*1.5 S2}" ls 2 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 aR-tree}" ls 8 lw 3 ps 2 with lines, file3 using 1:2 title "{/*1.5 Polyfit-3}" ls 7 lw 3 ps 2 with linespoints

# without S2
plot file2 using 1:2 title "{/*1.5 aR-tree}" ls 8 lw 3 ps 2 with lines, file3 using 1:2 title "{/*1.5 PolyFit-3}" lc 9 pt 13 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment2_Time_Erel/COUNT2D/plotcommand_2 <==
set term wxt size 600,450 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.5 relative error threshold}" offset 0,-0.5
set ylabel "{/*2.5 query response time (ns)}" offset -2.5,0
set ylabel rotate by 90
set tics font "Helvetica,18"

set logscale x
set logscale y

set lmargin 17.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT2D\\S2"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT2D\\aRtree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT2D\\Polyfit"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\COUNT2D\\MRTree"

set key spacing 2
#set key center right
set key at 0.18,210000
#set size ratio 0.8

set title "{/*2.5 Q_{rel}}" offset 0,-0.5

#plot file1 using 1:2 title "{/*2.0 S2}" ls 2 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*2.0 aR-tree}" ls 8 lw 3 ps 2 with lines, file4 using 1:2 title "{/*2.0 MRTree}" lc 7 pt 11 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*2.0 Polyfit-3}" ls 7 lw 3 ps 2 with linespoints

# without S2
plot file2 using 1:2 title "{/*2.0 aR-tree}" ls 8 lw 3 ps 2 with lines, file4 using 1:2 title "{/*2.0 MRTree}" lc 7 pt 11 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*2.0 PolyFit-3}" lc 9 pt 13 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment2_Time_Erel/MAX/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 relative error threshold}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"

#set yrange [0:300]
set logscale x
set logscale y

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\MAX\\aMaxTree"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\MAX\\Polyfit"

set key spacing 1.4
set key center right

set size square 1,1

plot file1 using 1:2 title "{/*1.5 aR-tree}" ls 8 lw 3 ps 2 with lines, file2 using 1:2 title "{/*1.5 PolyFit-1}" ls 6 pt 9 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment2_Time_Erel/MAX/plotcommand_2 <==
set style fill pattern 1 border
set xlabel "{/*2.0 relative error threshold}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"

#set yrange [0:300]
set logscale x
set logscale y

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\MAX\\aMaxTree"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment2_Time_Erel\\MAX\\Polyfit"

set key spacing 1.4
set key top right

set size square 1,1

plot file1 using 1:2 title "{/*1.5 aR-tree}" ls 1 lw 3 ps 2 with lines, file3 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment3_Time_MeasuredErel/COUNT1D/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 measured relative error (%)}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set logscale x
set xrange [0.01:10]
set logscale y
#unset logscale y

set grid ytics

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT1D\\entropyhist"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT1D\\stx"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT1D\\DBest"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT1D\\VerdictDB"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT1D\\polyfit"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT1D\\PLATO"

set key spacing 1.4
#set key at 0.08, 40000
#set key top left
set key outside
set key top right

set size square 1,1

plot file3 using 1:2 title "{/*1.5 DBest}" ls 12 pt 3 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 VerdictDB}" ls 13 pt 5 lw 3 ps 2 with linespoints, file6 using 1:2 title "{/*1.5 PLATO}" ls 13 pt 4 lw 3 ps 2, file1 using 1:2 title "{/*1.5 Hist}" ls 6 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 S-tree}" ls 2 pt 5 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment3_Time_MeasuredErel/COUNT1D/plotcommand_2 <==
set term wxt size 600,450 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.3 measured relative error (%)}" offset 0,-0.5
set ylabel "{/*2.5 query response time (ns)}" offset -2.5,0
set ylabel rotate by 90
set tics font "Helvetica,16"
set logscale x
set xrange [0.008:10]
set logscale y
#unset logscale y

set lmargin 16.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT1D\\entropyhist"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT1D\\stx"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT1D\\DBest"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT1D\\VerdictDB"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT1D\\polyfit"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT1D\\PLATO"


#set key off
set key spacing 1.6
set key at 0.15, 30000
#set key bottom left horizontal
#set size ratio 0.8

plot file3 using 1:2 title "{/*2.0 DBest}" ls 12 pt 10 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*2.0 VerdictDB}" ls 13 pt 5 lw 3 ps 2 with linespoints, file6 using 1:2 title "{/*2.0 PLATO}" ls 9 pt 1 lw 3 ps 2, file1 using 1:2 title "{/*2.0 Hist}" ls 6 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*2.0 S-tree}" ls 2 pt 12 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*2.0 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment3_Time_MeasuredErel/COUNT2D/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 measured relative error (%)}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set logscale x
set xtics ("0.5" 0.5, "1.0" 1.0, "5.0" 5.0, "10.0" 10.0)
set xrange [0.5:]
set logscale y
#unset logscale y

set grid ytics

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT2D\\DBest"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT2D\\VerdictDB"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT2D\\polyfit"

set key spacing 1.4
#set key top right
set key outside
set key top right

set size square 1,1

plot file3 using 1:2 title "{/*1.5 DBest}" ls 12 pt 3 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 VerdictDB}" ls 13 pt 5 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*1.5 PolyFit-3}" lc 9 pt 13 lw 3 ps 2 with linespoints



==> EDBT2021/Experiment3_Time_MeasuredErel/COUNT2D/plotcommand_2 <==
set term wxt size 600,450 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.5 measured relative error (%)}" offset 0,-0.5
set ylabel "{/*2.5 query response time (ns)}" offset -2.8,0
set ylabel rotate by 90
set tics font "Helvetica,18"
set logscale x
set xtics ("0.5" 0.5, "1.0" 1.0, "5.0" 5.0, "10.0" 10.0)
set xrange [0.4:]
set logscale y
#unset logscale y

set lmargin 17.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT2D\\DBest"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT2D\\VerdictDB"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment3_Time_MeasuredErel\\COUNT2D\\polyfit"

set key spacing 2.0
set key top right
#set size ratio 0.8

plot file3 using 1:2 title "{/*2.0 DBest}" ls 12 pt 10 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*2.0 VerdictDB}" ls 13 pt 5 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*2.0 PolyFit-3}" lc 9 pt 13 lw 3 ps 2 with linespoints



==> EDBT2021/Experiment4_Parameter_Eabs/COUNT1D_KB/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 structure size (KB)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xtics ("0" 0, "250" 250, "500" 500, "750" 750, "1000" 1000)
set xrange [0:*]


#set logscale x
set logscale y

set lmargin 14.5
#set rmargin 25.5
set rmargin 10.5
set tmargin 2.5
set bmargin 4.5

#file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_KB\\S2"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_KB\\FitingTree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_KB\\RMI"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_KB\\Polyfit"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_KB\\PGM"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_KB\\RadixSpline"


set key spacing 1.4
#set key center right
#set key at 950,100000

set key outside
set key top right

set size square 1,1


plot file3 using 1:2 title "{/*1.5 RMI}" ls 4 lw 3 ps 2 with linespoints, file6 using 1:2 title "{/*1.5 RadixSpline}" ls 10 lc 10 pt 6 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 FITing-Tree}" ls 3 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*1.5 PGM}" ls 8 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment4_Parameter_Eabs/COUNT1D_KB/plotcommand_2 <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 structure size (KB)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xtics ("0" 0, "250" 250, "500" 500, "750" 750, "1000" 1000)
set xrange [0:*]


#set logscale x
set logscale y

set lmargin 14.5
#set rmargin 25.5
set rmargin 10.5
set tmargin 2.5
set bmargin 4.5

#file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_KB\\S2"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_KB\\FitingTree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_KB\\RMI"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_KB\\Polyfit"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_KB\\PGM"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_KB\\RadixSpline"


set key spacing 1.4
set key center right
#set key at 950,100000


plot file3 using 1:2 title "{/*1.5 RMI}" ls 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 FITing-Tree}" ls 3 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*1.5 PGM}" ls 8 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment4_Parameter_Eabs/COUNT1D_MB/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 structure size (MB)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xtics ("0" 0, "250" 250, "500" 500, "750" 750, "1000" 1000)
set xrange [0:*]


#set logscale x
set logscale y

set lmargin 14.5
#set rmargin 25.5
set rmargin 10.5
set tmargin 2.5
set bmargin 4.5

#file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_MB\\S2"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_MB\\FitingTree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_MB\\RMI"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_MB\\Polyfit"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_MB\\PGM"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_MB\\RadixSpline"


set key spacing 1.4
set key center right

plot file3 using 1:2 title "{/*1.5 RMI}" ls 4 lw 3 ps 2 with linespoints, file6 using 1:2 title "{/*1.5 RadixSpline}" ls 10 lc 10 pt 6 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 FITing-Tree}" ls 3 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*1.5 PGM}" ls 8 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment4_Parameter_Eabs/COUNT1D_MB/plotcommand_2 <==
set style fill pattern 1 border
set xlabel "{/*2.0 deviation threshold {/Symbol d}}" offset 0,-0.5
set ylabel "{/*2.0 structure size (MB)}" offset 0,0
set ylabel rotate by 90
set tics font "Helvetica,18"
set xtics ("0" 0, "250" 250, "500" 500, "750" 750, "1000" 1000)
set xrange [0:*]

#set logscale x
set logscale y

set lmargin 12.5
set rmargin 10.5
set tmargin 2.5
set bmargin 4.5

#file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_MB\\S2"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_MB\\FitingTree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_MB\\RMI"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_MB\\PolyfitNew"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_MB\\PGM"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_MB\\RadixSpline"


set key spacing 2
set key center right

plot file3 using 1:2 title "{/*1.5 RMI}" ls 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 FITing-Tree}" ls 3 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*1.5 PGM}" ls 8 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment4_Parameter_Eabs/COUNT1D_Time_Size/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 query response time (ns)}" offset 0,-0.5
set ylabel "{/*2.0 index size (KB)}" offset 0,0
set ylabel rotate by 90
set tics font "Helvetica,18"
#set xtics ("0" 0, "250" 250, "500" 500, "750" 750, "1000" 1000)

#set logscale x
#set xrange [10:1000]

set xrange [0:*]

#set yrange [0:60]
set logscale y

set lmargin 12.5
set rmargin 10.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_Time_Size\\Polyfit"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_Time_Size\\FitingTree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment4_Parameter_Eabs\\COUNT1D_Time_Size\\PGM"

set key spacing 2
#set key top right
set key center right
#set key top center horizontal maxrows 1 maxcols 3

# set label for polyfit
set label "{/Symbol d} = 25" at 47,50 tc lt 7
set label "{/Symbol d} = 50" at 46,23.9 tc lt 7
set label "{/Symbol d} = 100" at 32,13.7 tc lt 7
set label "{/Symbol d} = 200" at 37,8.2 tc lt 7
set label "{/Symbol d} = 500" at 41,4.2 tc lt 7
set label "{/Symbol d} = 1000" at 70,2.5 tc lt 7

# set label for PGM
set label "{/Symbol d} = 25" at 85,46.736
set label "{/Symbol d} = 50" at 85,24.9
set label "{/Symbol d} = 100" at 82,12.2
set label "{/Symbol d} = 200" at 84,7.6
set label "{/Symbol d} = 500" at 92,4
set label "{/Symbol d} = 1000" at 119,2.240

# set label for FITingTree
set label "{/Symbol d} = 25" at 160,134.6 tc lt 3
set label "{/Symbol d} = 50" at 157,56 tc lt 3
set label "{/Symbol d} = 100" at 134,28.204 tc lt 3
set label "{/Symbol d} = 200" at 140,16.2 tc lt 3
set label "{/Symbol d} = 500" at 145,7.532 tc lt 3
set label "{/Symbol d} = 1000" at 245,3.9 tc lt 3

set title "{/*2.0 Q_{rel}}" offset 0,-0.5

plot file1 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PGM}" ls 8 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 FITing-Tree}" ls 3 lw 3 ps 2 with linespoints



==> EDBT2021/Experiment5_ConstructionTime/vary_Eabs(legacy)/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 construction time (s)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_Eabs\\Polyfit1"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_Eabs\\Polyfit2"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_Eabs\\Polyfit3"

set key spacing 1.4
set key top left

#plot file1 using 1:2 title "{/*1.5 Polyfit-1}" ls 2 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 Polyfit-2}" ls 3 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 Polyfit-3}" ls 4 lw 3 ps 2 with linespoints

plot file1 using 1:2 title "{/*1.5 PolyFit-1}" ls 6 lw 3 ps 2 pt 9 with linespoints, file2 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-3}" ls 9 lw 3 ps 2 pt 13 with linespoints

==> EDBT2021/Experiment5_ConstructionTime/vary_dataset_size/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 dataset size (million records)}" offset 0,-0.3
set ylabel "{/*2.0 construction time (s)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xrange [0:*]

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\Polyfit"

set key spacing 1.4
set key top left 

set size square 1,1

plot file1 using 1:2 title "{/*1.5 PolyFit-OSM (1Dim)}" ls 6 lw 3 ps 2 pt 7 with linespoints

==> EDBT2021/Experiment5_ConstructionTime/vary_dataset_size/plotcommand_2 <==
set term wxt size 450,350 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.0 dataset size (million records)}" offset 0,-0.3
set ylabel "{/*2.0 construction time (s)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xrange [0:*]
set logscale y

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\Polyfit"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\Polyfit2d"

set key spacing 1.4
set key top right 

#set size square 1,1

# for 1dim
plot file1 using 1:2 title "{/*1.5 PolyFit-2}" ls 6 lw 3 ps 2 pt 7 with linespoints

# for 2dim
#plot file2 using 1:2 title "{/*1.5 PolyFit-3}" ls 7 lw 3 ps 2 pt 9 with linespoints

==> EDBT2021/Experiment5_ConstructionTime/vary_dataset_size/plotcommand_compare <==
set term wxt size 450,350 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.0 dataset size (million records)}" offset 0,-0.3
set ylabel "{/*2.0 construction time (s)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xrange [0:*]
set logscale y

set lmargin 14.5
set rmargin 24.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\Polyfit"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\FITingTree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\PGM"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\PLATO"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\RMI"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\ARTree"
file7 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\MRTree"
file8 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\Hist"
file9 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\DBest"

set key spacing 1.4
set key outside
set key top right 

#set size square 1,1

# for 1dim
plot file8 using 1:2 title "{/*1.5 Hist}" ls 6 lw 3 ps 2 with linespoints, file9 using 1:2 title "{/*1.5 DBest}" ls 12 pt 10 lw 3 ps 2 with linespoints, file1 using 1:2 title "{/*1.5 PolyFit-2}" ls 6 lw 3 ps 2 pt 7 with linespoints, file5 using 1:2 title "{/*1.5 RMI}" ls 4 lw 3 ps 2 with linespoints, file7 using 1:2 title "{/*1.5 MRTree}" lc 7 pt 11 lw 3 ps 2 with linespoints, file6 using 1:2 title "{/*1.5 aR-tree}" ls 8 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 PLATO}" ls 9 pt 1 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 FITing-tree}" ls 3 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PGM}" ls 8 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment5_ConstructionTime/vary_dataset_size/plotcommand_compare2d <==
set term wxt size 450,350 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.0 dataset size (million records)}" offset 0,-0.3
set ylabel "{/*2.0 construction time (s)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xrange [0:*]
set logscale y

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

set lmargin 14.5
set rmargin 20.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\Polyfit2d"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\ARTree2d"
file7 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\MRTree2d"
file9 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_dataset_size\\DBest2d"

set key spacing 1.4
set key outside
set key top right 

#set size square 1,1

# for 1dim
plot file9 using 1:2 title "{/*1.5 DBest}" ls 12 pt 10 lw 3 ps 2 with linespoints, file1 using 1:2 title "{/*1.5 PolyFit-3}" ls 6 lw 3 ps 2 pt 7 with linespoints, file7 using 1:2 title "{/*1.5 MRTree}" lc 7 pt 11 lw 3 ps 2 with linespoints, file6 using 1:2 title "{/*1.5 aR-tree}" ls 8 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment5_ConstructionTime/vary_degree/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 degree}" offset 0,-0.3
set ylabel "{/*2.0 construction time (s)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xtics ("1" 1, "2" 2, "3" 3, "4" 4)
set xrange [1:*]

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_degree\\Polyfit"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_degree\\Polyfit2d"

set key spacing 1.4
set key top right

set size square 1,1

plot file2 using 1:2 title "{/*1.5 PolyFit-OSM (2Dim)}" ls 7 lw 3 ps 2 pt 9 with linespoints, file1 using 1:2 title "{/*1.5 PolyFit-TWEET (1Dim)}" ls 6 lw 3 ps 2 pt 7 with linespoints

==> EDBT2021/Experiment5_ConstructionTime/vary_degree/plotcommand_2 <==
set term wxt size 450,350 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.0 degree}" offset 0,-0.3
set ylabel "{/*2.0 construction time (s)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xtics ("1" 1, "2" 2, "3" 3, "4" 4)
set xrange [1:*]
set logscale y

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_degree\\Polyfit"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment5_ConstructionTime\\vary_degree\\Polyfit2d"

set key spacing 1.4
set key top right 

#set size square 1,1

# for 1dim
#plot file1 using 1:2 title "{/*1.5 PolyFit}" ls 6 lw 3 ps 2 pt 7 with linespoints

# for 2dim
plot file2 using 1:2 title "{/*1.5 PolyFit}" ls 7 lw 3 ps 2 pt 9 with linespoints

# for both
#plot file2 using 1:2 title "{/*1.5 PolyFit-OSM (2Dim)}" ls 7 lw 3 ps 2 pt 9 with linespoints, file1 using 1:2 title "{/*1.5 PolyFit-TWEET (1Dim)}" ls 6 lw 3 ps 2 pt 7 with linespoints

==> EDBT2021/Experiment6_Time_degree_Eabs/COUNT1D/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xtics ("0" 0, "250" 250, "500" 500, "750" 750, "1000" 1000)
#set logscale x
set logscale y
set xrange[0:]

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

#file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT1D\\FitingTree"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT1D\\Polyfit1"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT1D\\Polyfit2"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT1D\\Polyfit3"

set key spacing 1.4
# set key top right
set key outside
set key top right

set size square 1,1

#plot file1 using 1:2 title "{/*1.5 FITing-Tree}" ls 2 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 Polyfit-1}" ls 3 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 Polyfit-2}" ls 4 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 Polyfit-3}" ls 6 lw 3 ps 2 with linespoints

plot file2 using 1:2 title "{/*1.5 PolyFit-1}" ls 6 lw 3 ps 2 pt 9 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-3}" ls 9 lw 3 ps 2 pt 13 with linespoints

==> EDBT2021/Experiment6_Time_degree_Eabs/COUNT1D/plotcommand_2 <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xtics ("0" 0, "250" 250, "500" 500, "750" 750, "1000" 1000)
#set logscale x
set logscale y
set xrange[0:]

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT1D\\Polyfit1"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT1D\\Polyfit2"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT1D\\Polyfit3"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT1D\\Polyfit4"

set key spacing 1.4
set key top right
#set size ratio 0.8

plot file1 using 1:2 title "{/*1.5 PolyFit-1}" ls 6 lw 3 ps 2 pt 9 with linespoints, file2 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-3}" ls 9 lw 3 ps 2 pt 13 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-4}" ls 15 lc 4 lw 3 ps 2 pt 17 with linespoints

==> EDBT2021/Experiment6_Time_degree_Eabs/COUNT1D_varydeg/plotcommand <==
#set term pdf enhanced mono lw 4 font "Helvetica,36pt" size 8,6

set term wxt size 600,450 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.5 degree}" offset 0,-0.3
set ylabel "{/*2.5 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,18"
set xtics ("1" 1, "2" 2, "3" 3, "4" 4)
#set logscale x
#set logscale y
set xrange[1:]
set yrange[0:]

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT1D_varydeg\\100"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT1D_varydeg\\200"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT1D_varydeg\\500"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT1D_varydeg\\1000"

set key spacing 2
set key bottom right

set title "{/*2.5 Q_{abs}}" offset 0,-0.5

# plot all
#plot file1 using 1:2 title "{/*2.0 {/Symbol e}_{abs}=100}" ls 9 lc 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*2.0 {/Symbol e}_{abs}=200}" ls 3 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*2.0 {/Symbol e}_{abs}=500}" ls 10 pt 4 lc 2 lw 3 ps 2 with linespoints

# only default
plot file1 using 1:2 title "{/*2.0 {/Symbol e}_{abs}=100}" ls 9 lc 4 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment6_Time_degree_Eabs/COUNT2D/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xtics ("0" 0, "250" 250, "500" 500, "750" 750, "1000" 1000)
#set logscale x
#set logscale y
set xrange[0:]

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT2D\\Polyfit2"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT2D\\Polyfit3"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT2D\\Polyfit4"

set key spacing 1.4
# set key top right
set key outside
set key top right

set size square 1,1


#plot file1 using 1:2 title "{/*1.5 FITing-Tree}" ls 2 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 Polyfit-1}" ls 3 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 Polyfit-2}" ls 4 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 Polyfit-3}" ls 6 lw 3 ps 2 with linespoints

plot file2 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-3}" ls 9 lw 3 ps 2 pt 13 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-4}" ls 15 lc 4 lw 3 ps 2 pt 17 with linespoints

==> EDBT2021/Experiment6_Time_degree_Eabs/COUNT2D/plotcommand_2 <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xtics ("0" 0, "250" 250, "500" 500, "750" 750, "1000" 1000)
#set logscale x
set logscale y
set xrange[0:]

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT2D\\Polyfit1"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT2D\\Polyfit2"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT2D\\Polyfit3"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT2D\\Polyfit4"

set key spacing 1.4
set key center right
set size ratio 0.8


plot file1 using 1:2 title "{/*1.5 PolyFit-1}" ls 6 lw 3 ps 2 pt 9 with linespoints, file2 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-3}" ls 9 lw 3 ps 2 pt 13 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-4}" ls 15 lc 4 lw 3 ps 2 pt 17 with linespoints

==> EDBT2021/Experiment6_Time_degree_Eabs/COUNT2D_varydeg/plotcommand <==
set term wxt size 600,450 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.5 degree}" offset 0,-0.3
set ylabel "{/*2.5 query response time (ns)}" offset -2.5,0
set ylabel rotate by 90
set tics font "Helvetica,18"
set xtics ("1" 1, "2" 2, "3" 3, "4" 4)
#set logscale x
#set logscale y
set xrange[1:]
set yrange[0:]

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT2D_varydeg\\100"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT2D_varydeg\\200"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\COUNT2D_varydeg\\500"

set key spacing 2
set key bottom right

set title "{/*2.5 Q_{abs}}" offset 0,-0.5

# plot all
#plot file1 using 1:2 title "{/*2.0 {/Symbol e}_{abs}=100}" ls 9 lc 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*2.0 {/Symbol e}_{abs}=200}" ls 3 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*2.0 {/Symbol e}_{abs}=500}" ls 10 pt 4 lc 2 lw 3 ps 2 with linespoints

# only default
plot file1 using 1:2 title "{/*2.0 {/Symbol e}_{abs}=100}" ls 9 lc 4 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment6_Time_degree_Eabs/MAX/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"

set xtics ("0" 0, "250" 250, "500" 500, "750" 750, "1000" 1000)
set xrange[0:]
#set logscale x
#set logscale y

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\MAX\\Polyfit"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\MAX\\Polyfit2"

set key spacing 1.4
# set key bottom left
set key outside
set key top right

set size square 1,1

#plot file2 using 1:2 title "{/*1.5 PolyFit-1}" ls 6 lw 3 ps 2 pt 9 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-3}" ls 9 lw 3 ps 2 pt 13 with linespoints

plot file2 using 1:2 title "{/*1.5 PolyFit-1}" ls 6 lw 3 ps 2 pt 9 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment6_Time_degree_Eabs/MAX/plotcommand_2 <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 query response time (ns)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"

set xtics ("0" 0, "250" 250, "500" 500, "750" 750, "1000" 1000)
set xrange[0:]
#set logscale x
set logscale y

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\MAX\\Polyfit"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\MAX\\Polyfit2"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\MAX\\Polyfit3"

set key spacing 1.4
set key bottom right
set size ratio 0.8


plot file1 using 1:2 title "{/*1.5 PolyFit-1}" ls 6 lw 3 ps 2 pt 9 with linespoints, file2 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-3}" ls 9 lw 3 ps 2 pt 13 with linespoints

==> EDBT2021/Experiment6_Time_degree_Eabs/MAX_varydeg/plotcommand <==
set term wxt size 600,450 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.5 degree}" offset 0,-0.3
set ylabel "{/*2.5 query response time (ns)}" offset -1.5,0
set ylabel rotate by 90
set tics font "Helvetica,18"
set xtics ("1" 1, "2" 2, "3" 3)
#set logscale x
#set logscale y
set xrange[1:]
set yrange[0:]

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\MAX_varydeg\\100"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\MAX_varydeg\\200"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment6_Time_degree_Eabs\\MAX_varydeg\\500"

set key spacing 2
set key bottom right

set title "{/*2.5 Q_{abs}}" offset 0,-0.5

# all
#plot file1 using 1:2 title "{/*2.0 {/Symbol e}_{abs}=100}" ls 9 lc 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*2.0 {/Symbol e}_{abs}=200}" ls 3 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*2.0 {/Symbol e}_{abs}=500}" ls 10 pt 4 lc 2 lw 3 ps 2 with linespoints

# only default
plot file1 using 1:2 title "{/*2.0 {/Symbol e}_{abs}=100}" ls 9 lc 4 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment7_Eabs_Segmentations/COUNT1D/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 segment amount}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xrange [0:*]

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\Polyfit1"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\Polyfit2"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\Polyfit3"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\FitingTree"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\dogulas"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\PGM"
file7 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\RadixSpline"

set key spacing 1.4
set key top right

plot file5 using 1:2 title "{/*1.5 Dogulas}" ls 9 lc 4 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 FITingTree}" ls 3 lw 3 ps 2 with linespoints, file7 using 1:2 title "{/*1.5 RadixSpline}" ls 10 pt 4 lc 2 lw 3 ps 2 with linespoints, file6 using 1:2 title "{/*1.5 PGM}" ls 8 lw 3 ps 2 pt 9 with linespoints, file2 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-3}" ls 9 lw 3 ps 2 pt 13 with linespoints

==> EDBT2021/Experiment7_Eabs_Segmentations/COUNT1D/plotcommand_2 <==
set style fill pattern 1 border
set xlabel "{/*2.0 deviation threshold {/Symbol d}}" offset 0,-0.3
set ylabel "{/*2.0 # of segments}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xrange [0:*]

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\Polyfit1"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\Polyfit2"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\Polyfit3"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\FitingTree"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\dogulas"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\PGM"
file7 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\RadixSpline"

set key spacing 1.4
set key top right

plot file4 using 1:2 title "{/*1.5 FITingTree}" ls 3 lw 3 ps 2 with linespoints, file6 using 1:2 title "{/*1.5 PGM}" ls 8 lw 3 ps 2 pt 9 with linespoints, file2 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment7_Eabs_Segmentations/COUNT1D/plotcommand_models <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 model amount}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xrange [0:*]

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\Polyfit1"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\Polyfit2"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\Polyfit3"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\FitingTree"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\dogulas"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\PGM"
file7 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT1D\\RadixSpline"

set key spacing 1.4
set key top right

plot file4 using 1:2 title "{/*1.5 FITingTree}" ls 3 lw 3 ps 2 with linespoints, file7 using 1:2 title "{/*1.5 RadixSpline}" ls 10 pt 4 lc 2 lw 3 ps 2 with linespoints, file6 using 1:2 title "{/*1.5 PGM}" ls 8 lw 3 ps 2 pt 9 with linespoints, file2 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-3}" ls 9 lw 3 ps 2 pt 13 with linespoints

==> EDBT2021/Experiment7_Eabs_Segmentations/COUNT2D/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 model amount}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xrange [0:*]

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5


file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT2D\\Polyfit2"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT2D\\Polyfit3"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT2D\\Polyfit4"

set key spacing 1.4
set key top right

plot file2 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-3}" ls 9 lw 3 ps 2 pt 13 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-4}" ls 15 lc 4 lw 3 ps 2 pt 17 with linespoints

==> EDBT2021/Experiment7_Eabs_Segmentations/COUNT2D/plotcommand_2 <==
set style fill pattern 1 border
set xlabel "{/*2.0 deviation threshold {/Symbol d}}" offset 0,-0.3
set ylabel "{/*2.0 # of segments}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xrange [0:*]
set yrange [0:100000]
#set logscale y
set ytics ("0" 0, "20000" 20000, "40000" 40000, "60000" 60000, "80000" 80000, "100000" 100000)

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5


file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT2D\\Polyfit2"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT2D\\Polyfit3"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\COUNT2D\\Polyfit4"

set key spacing 1.4
set key top right

plot file2 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-3}" ls 9 lw 3 ps 2 pt 13 with linespoints, file4 using 1:2 title "{/*1.5 PolyFit-4}" ls 15 lc 4 lw 3 ps 2 pt 17 with linespoints

==> EDBT2021/Experiment7_Eabs_Segmentations/plotcommand_models <==
set style fill pattern 1 border
set xlabel "{/*2.0 absolute error threshold}" offset 0,-0.3
set ylabel "{/*2.0 model amount}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\Polyfit1"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\Polyfit2"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\Polyfit3"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\FitingTree"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\dogulas"
file6 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\PGM"
file7 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment7_Eabs_Segmentations\\RadixSpline"

set key spacing 1.4
set key top right

#plot file1 using 1:2 title "{/*1.5 Polyfit-1}" ls 2 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 Polyfit-2}" ls 3 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 Polyfit-3}" ls 4 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 FITingTree}" ls 5 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*1.5 Dogulas}" ls 6 lw 3 ps 2 with linespoints

plot file5 using 1:2 title "{/*1.5 Dogulas}" ls 9 lc 2 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*1.5 FITingTree}" ls 4 lw 3 ps 2 with linespoints, file1 using 1:2 title "{/*1.5 PolyFit-1}" ls 6 lw 3 ps 2 pt 9 with linespoints, file2 using 1:2 title "{/*1.5 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 PolyFit-3}" ls 9 lw 3 ps 2 pt 13 with linespoints

==> EDBT2021/Experiment8_Eabs_HitRate/COUNT1D/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 relative error threshold}" offset 0,-0.3
set ylabel "{/*2.0 hit percentage (%)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xtics ("0.005" 0.005, "0.01" 0.01, "0.05" 0.05, "0.1" 0.1, "0.2" 0.2)
set logscale x

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\COUNT1D\\100"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\COUNT1D\\200"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\COUNT1D\\500"

set key spacing 1.4
#set key bottom right

set key outside
set key top right

set size square 1,1

set termopt enhanced

plot file1 using 1:2 title "{/*1.5 {/Symbol e}_{abs}=100}" ls 9 lc 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 {/Symbol e}_{abs}=200}" ls 3 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 {/Symbol e}_{abs}=500}" ls 10 pt 4 lc 2 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment8_Eabs_HitRate/COUNT1D/plotcommand_2 <==
set term wxt size 600,450 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.5 relative error threshold}" offset 0,-0.5
set ylabel "{/*2.5 hit percentage (%)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,18"
set xtics ("0.005" 0.005, "0.01" 0.01, "0.05" 0.05, "0.1" 0.1, "0.2" 0.2)
set logscale x
set xrange[0.004:*]

set lmargin 12.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\COUNT1D\\100"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\COUNT1D\\200"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\COUNT1D\\500"

set key spacing 2.0
set key center right
#set size ratio 0.8

set termopt enhanced

plot file1 using 1:2 title "{/*2.0 {/Symbol d}=100}" ls 9 lc 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*2.0 {/Symbol d}=200}" ls 3 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*2.0 {/Symbol d}=500}" ls 10 pt 4 lc 2 lw 3 ps 2 with linespoints

# plot black and white
#plot file1 using 1:2 title "{/*1.5 {/Symbol d}=100}" ls 9 lc 0 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 {/Symbol d}=200}" ls 3 lc 0 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 {/Symbol d}=500}" ls 10 lc 0 pt 4 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment8_Eabs_HitRate/COUNT2D/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 relative error threshold}" offset 0,-0.3
set ylabel "{/*2.0 hit percentage (%)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xtics ("0.005" 0.005, "0.01" 0.01, "0.05" 0.05, "0.1" 0.1, "0.2" 0.2)
set logscale x

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\COUNT2D\\100"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\COUNT2D\\500"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\COUNT2D\\1000"


set key spacing 1.4
#set key bottom right

set key outside
set key top right

set size square 1,1

plot file1 using 1:2 title "{/*1.5 {/Symbol e}_{abs}=100}" ls 9 lc 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 {/Symbol e}_{abs}=500}" ls 3 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 {/Symbol e}_{abs}=1000}" ls 10 pt 4 lc 2 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment8_Eabs_HitRate/COUNT2D/plotcommand_2 <==
set term wxt size 600,450 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.5 relative error threshold}" offset 0,-0.5
set ylabel "{/*2.5 hit percentage (%)}" offset -2.0,0
set ylabel rotate by 90
set tics font "Helvetica,18"
set xtics ("0.005" 0.005, "0.01" 0.01, "0.05" 0.05, "0.1" 0.1, "0.2" 0.2)
set logscale x
set xrange[0.004:*]

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\COUNT2D\\100"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\COUNT2D\\500"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\COUNT2D\\1000"

set key spacing 2.0
set key center right
#set size ratio 0.8

plot file1 using 1:2 title "{/*2.0 {/Symbol d}=100}" ls 9 lc 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*2.0 {/Symbol d}=500}" ls 3 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*2.0 {/Symbol d}=1000}" ls 10 pt 4 lc 2 lw 3 ps 2 with linespoints

#plot black and white
#plot file1 using 1:2 title "{/*1.5 {/Symbol d}=100}" ls 9 lc 0 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 {/Symbol d}=500}" ls 3 lc 0 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 {/Symbol d}=1000}" ls 10 lc 0 pt 4 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment8_Eabs_HitRate/MAX/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 relative error threshold}" offset 0,-0.3
set ylabel "{/*2.0 hit percentage (%)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xtics ("0.005" 0.005, "0.01" 0.01, "0.05" 0.05, "0.1" 0.1, "0.2" 0.2)
set logscale x

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\MAX\\100"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\MAX\\200"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\MAX\\500"


set key spacing 1.4
#set key bottom right

set key outside
set key top right

set size square 1,1

set termopt enhanced

plot file1 using 1:2 title "{/*1.5 {/Symbol e}_{abs}=100}" ls 9 lc 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 {/Symbol e}_{abs}=200}" ls 3 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 {/Symbol e}_{abs}=500}" ls 10 pt 4 lc 2 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment8_Eabs_HitRate/MAX/plotcommand_2 <==
set term wxt size 600,450 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.5 relative error threshold}" offset 0,-0.5
set ylabel "{/*2.5 hit percentage (%)}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,18"
set xtics ("0.005" 0.005, "0.01" 0.01, "0.05" 0.05, "0.1" 0.1, "0.2" 0.2)
set logscale x
set xrange[0.004:*]

set lmargin 12.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\MAX\\100"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\MAX\\200"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\MAX\\500"

set key spacing 2.0
set key center right
#set size ratio 0.8

set termopt enhanced

plot file1 using 1:2 title "{/*2.0 {/Symbol d}=100}" ls 9 lc 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*2.0 {/Symbol d}=200}" ls 3 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*2.0 {/Symbol d}=500}" ls 10 pt 4 lc 2 lw 3 ps 2 with linespoints

# plot black and white
#plot file1 using 1:2 title "{/*1.5 {/Symbol d}=100}" ls 9 lc 0 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 {/Symbol d}=200}" ls 3 lc 0 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 {/Symbol d}=500}" ls 10 lc 0 pt 4 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment8_Eabs_HitRate/plotcommand <==
set style fill pattern 1 border
set xlabel "{/*2.0 relative error threshold}" offset 0,-0.3
set ylabel "{/*2.0 hit percentage}" offset -1,0
set ylabel rotate by 90
set tics font "Helvetica,14"
set xtics ("0.005" 0.005, "0.01" 0.01, "0.05" 0.05, "0.1" 0.1, "0.2" 0.2)
set logscale x

set yrange [80:*]

set lmargin 14.5
set rmargin 4.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\COUNT1D"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\COUNT2D"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment8_Eabs_HitRate\\MAX1D"


set key spacing 1.4
set key bottom right

plot file1 using 1:2 title "{/*1.5 COUNT-1D}" ls 9 lc 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*1.5 COUNT-2D}" ls 3 lw 3 ps 2 with linespoints, file3 using 1:2 title "{/*1.5 MAX-1D}" ls 10 pt 4 lc 2 lw 3 ps 2 with linespoints

==> EDBT2021/Experiment9_Selectivity/COUNT1D/plotcommand <==
set term wxt size 600,450 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.5 selectivity (%)}" offset 0,-0.5
set ylabel "{/*2.5 query response time (ns)}" offset -2.5,0
set ylabel rotate by 90
set tics font "Helvetica,18"

set xrange [0.008:10]

set logscale x
set logscale y

set lmargin 15.5
set rmargin 10.5
set tmargin 2.5
set bmargin 4.5

file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment9_Selectivity\\COUNT1D\\FitingTree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment9_Selectivity\\COUNT1D\\RMI"
file4 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment9_Selectivity\\COUNT1D\\Polyfit"
file5 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment9_Selectivity\\COUNT1D\\PGM"
file7 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment9_Selectivity\\COUNT1D\\MRTree"
file8 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment9_Selectivity\\COUNT1D\\aRtree"

#set key off
set key spacing 1.4
set key top center horizontal
#set size ratio 0.8

set title "{/*2.5 Q_{abs}}" offset 0,-0.2

# COMPARE WITHOUT SAMPLING
plot file7 using 1:2 title "{/*2.0 MRTree}" lc 7 pt 11 lw 3 ps 2 with linespoints, file8 using 1:2 title "{/*2.0 aR-tree}" ls 8 lw 3 ps 2 with lines, file3 using 1:2 title "{/*2.0 RMI}" ls 4 lw 3 ps 2 with linespoints, file2 using 1:2 title "{/*2.0 FITing-Tree}" ls 3 lw 3 ps 2 with linespoints, file5 using 1:2 title "{/*2.0 PGM}" ls 8 lw 3 ps 2 with linespoints, file4 using 1:2 title "{/*2.0 PolyFit-2}" ls 7 lw 3 ps 2 with linespoints


==> EDBT2021/Experiment9_Selectivity/COUNT2D/plotcommand <==
set term wxt size 600,450 # default is 640*384 

set style fill pattern 1 border
set xlabel "{/*2.5 selectivity (%)}" offset 0,-0.5
set ylabel "{/*2.5 query response time (ns)}" offset -2.5,0
set ylabel rotate by 90
set tics font "Helvetica,18"

set xrange [0.008:10]

set logscale x
set logscale y

set lmargin 15.5
set rmargin 10.5
set tmargin 2.5
set bmargin 4.5

file1 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment9_Selectivity\\COUNT2D\\Polyfit"
file2 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment9_Selectivity\\COUNT2D\\MRTree"
file3 = "D:\\Polyfit_experiments\\EDBT2021\\Experiment9_Selectivity\\COUNT2D\\aRtree"

#set key off
set key spacing 2.0
set key top left
#set size ratio 0.8

set title "{/*2.5 Q_{abs}}" offset 0,-0.2

# COMPARE WITHOUT SAMPLING
plot file3 using 1:2 title "{/*2.0 aR-tree}" ls 8 lw 3 ps 2 with lines, file2 using 1:2 title "{/*2.0 MRTree}" lc 7 pt 11 lw 3 ps 2 with linespoints, file1 using 1:2 title "{/*2.0 PolyFit-3}" ls 7 lw 3 ps 2 with linespoints


==> case_2d.tex <==
\section{Extensions for Queries with Multiple keys}
\label{sec:extend_2d}%
In previous sections, we mainly focus on range aggregate queries, in which each element only contains one single key (cf. Definition \ref{def:RAQ}). However, existing work \cite{heimel2015self,riondato2011vc,gunopulos2005selectivity,gunopulos2000approximating} also support range aggregate queries with two keys for each element. In this section, we discuss how to extend our techniques in this setting (cf. Definition \ref{def:2D_Approx_RAQ}). As a remark, our techniques can be also extended to the setting of multiple keys. Here, we only focus on count query. However, we can also adopt our methods for other types of range aggregate queries.



\subsection{Index Construction} \label{sec:2D_construct}


\begin{figure}[!hbt]
\center
\includegraphics[width=0.8\columnwidth]{figures/Accu2D_LinearSurface_2500_BR.pdf}
\caption{Blue dots are the data points from the Twitter dataset \cite{chen2015temporal} (x-axis: latitude and y-axis: cumulative number of tweets), $LR(x)$, $LS(x)$ and $\mathbb{P}(x)$ are linear regression, linear segment and polynomial functions respectively.}
\label{fig:idea2D}
\end{figure}



\begin{definition}
\label{def:2D_Approx_RAQ}
Given $\mathcal{D}$ as a set of elements $(u, v, w)$, where $u$, $v$ and $w$ are the first key, second key and the weight respectively, and the ranges of keys are $[L_1, U_1]$ for $u$ and $[L_2, U_2]$ for $v$, we define $\mathcal{D}[L_1,U_1][L_2,U_2]$ as the subset of $\mathcal{D}$ such that all the keys $(u,v)$ are within the above region, i.e.,
\begin{equation*}
\mathcal{D}[L_1,U_1][L_2,U_2]=\sigma_{u\in [L_1,U_1], v\in [L_2,U_2]} (\mathcal{D})
\end{equation*}
The count query is defined as:
\begin{equation}
\label{eq:2D_count}
R_{sum}(\mathcal{D},[L_1,U_1][L_2,U_2])=|\mathcal{D}[L_1,U_1][L_2,U_2]|
\end{equation}
\end{definition}

Instead of building the key-cumulative array (cf. Figure \ref{fig:key_cumulative_array}) for solving the count query, we build the following key-cumulative function to represent the surface (cf. Figure \ref{fig:example2D}), which are formally stated in Definition \ref{def:accu2D}.
%


\begin{definition}
%\vspace{-2mm}
\label{def:accu2D}
The key-cumulative function with two keys for count query is defined as $CF_{sum}(u,v)$, where:
\begin{eqnarray}
\label{eq:accu2d}
CF_{sum}(u,v) = R_{sum}(\mathcal{D},[-\infty, u][-\infty, v])
\end{eqnarray}
\end{definition}

Therefore, we can solve the count query $R_{sum}(\mathcal{D},[L_1,U_1][L_2,U_2])$, using the following equation.
\begin{equation*}
\begin{split}
R_{sum}(\mathcal{D},[L_1,U_1][L_2,U_2])=CF_{sum}(L_2,U_2)-CF_{sum}(L_2,U_1)\\
-CF_{sum}(L_1,U_2)+CF_{sum}(L_1,U_1)
\end{split}
\end{equation*}

Then, we follow the similar idea in Section \ref{sec:min_error} and utilize the polynomial surface $\mathbb{P}(u,v)$ to approximate the key cumulative function $CF_{sum}(u,v)$ with two keys, where:
$$\mathbb{P}(u,v)=\sum_{i=1,i+j\leq deg}^{deg} a_{i,j} u^i v^j$$

By replacing $F(k_i)$ and $\mathbb{P}(k_i)$ in Equation \ref{eq:error} by $F(u_i,v_i)$ and $\mathbb{P}(u_i,v_i)$ respectively, we can obtain the similar linear programming problem for obtaining the best parameters $a_{i,j}$. However, unlike the one-dimensional case, it takes $O(n^2)$ to obtain the minimum number of segmentations by using the GS method (cf. Section \ref{sec:GS}), which is infeasible even for small-scale dataset (e.g., 10000 points). As such, we propose to utilize the Quad-tree based solution to obtain the segmentation. Observe from Figure \ref{fig:quad_tree}, once the segment does not fulfill the error guarantee $\delta$ (e.g., white rectangles), we continuously break each of these white rectangles into four rectangles in each iteration. Our method terminates when all rectangles fulfill the error guarantee $\delta$.

\begin{figure}[!hbt]
\center
\includegraphics[width=1.0\columnwidth,page=1]{figures/2DDivide_crop_v2.pdf}
\caption{Quad-tree based approach for obtaining the segmentation}
\label{fig:quad_tree}
\end{figure} 


\subsection{Query Methods} \label{sec:2D_query}
%

++ discuss adaptations of query methods for the 2D case




==> exper.tex <==
\section {Experiment}

In this section, we empirically study Polyfit. In summary, we answer the following questions:

\begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
	\item How the hyper-parameters (relative error threshold and absolute error threshold) affect the performance of our solution and how to set the best absolute error threshold (Section \ref{sec:hypertune}).
	\item How good is our method compared with FITingTree, RMI and other traditional statistical methods (Section \ref{sec:performance}).
	\item Why our segmentation method is necessary and how good it is(Section \ref{sec:whyoptseg}).
	\item Other features of our method including robustness to scale, construction time and accuracy-space trade off (Section \ref{sec:otherfeatures}).
\end{enumerate}

\subsection{Experimental Setting}
\label{sec:expsetting}
\subsubsection{Environments}
All the experiments in this section are written in C++ and conducted in Windows 10 platform with Intel Core i7-8700 processor, 32GB memory, under -O2 compiling optimization provided by visual studio 2017.

\subsubsection{Datasets and Query Sets}

We use 3 real datasets from different domains to evaluate the performance of our method under variety realistic data distribution.

% \usepackage{enumitem} % for experiment section
\begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
	\item TWEET: The tweet dataset \cite{chen2015temporal} contains 1 million tweets collected from April to October in 2012 worldwide. We use latitude to index this dataset for our 1D count query.  We use the this dataset as the default dataset in parameter tunning, segmentation comparison and feature evaluation.
	\item OSM: The OpenStreetMap dataset \cite{osmplanet2019} has been widely used in previous literatures. In this experiment, we randomly select 100M records under its 2019 package and use the latitude (and longitude) for our count query under 1D (and 2D) settings. We use this dataset in scaling and 2D performance comparison.
	\item HKI: The Hong Kong 40 Index of 2018 \cite{hk40index} is a time-series dataset recording the index value in minute level, which adds up to 0.9M records in total. We use this dataset to evaluate the min/max query performance of our method.
\end{enumerate}

For each dataset, we randomly generate 1000 queries. For the OSM dataset, another 1000 queries are generated for 2D experiments. Specifically, for 1D query, the lower and upper query keys are randomly picked from the keys in the corresponding dataset. For 2D query, the query length in each dimension follows the Gaussian distribution with $\mu=0$ and $\sigma=10\%$ of the domain size. Since COUNT/SUM/AVG queries share the same property in index construction and query processing, we use COUNT to represent this category and MAX to represent the rest in this experiment.

\subsubsection{List of Comparative Techniques}

\begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
	\item Hist: The state-of-the-art entropy-based histogram optimized for range selectivity query \cite{to2013entropy}. When query, we first locate the related buckets, then calculate the required statistic info.
	\item STX: The STX method builds an STX B+ tree \cite{STXBtree} for the sorted key-value pairs, then the COUNT/SUM query is equivalent to two exact searches using the index. This method could be combined with sampling to balance the query response time and accuracy.
	\item S2: The S2 sampling algorithm \cite{haas1992sequential}, which is able to guarantee any relative error threshold under a given probability.
	\item RMI: Recursive model index \cite{kraska2018case}. The aggregate query procedure is using RMI is the same as STX (without sampling).
	\item FITing-Tree: FITingTree index \cite{journals/corr/abs-1801-10207}. The aggregate query procedure is using FITing-Tree is the same as STX (without sampling). When compared with our solution, we also perform the filter-refinement procedures to guarantee relative error by default.
	\item Dogulas: The well-known Dogulas-Peucker algorithm. We use it as one of the comparison baseline for segmentation.
	\item aRtree: The aggregate Rtree, which store the local COUNT info in each node. We used it for 2D COUNT query comparison. The implement is based on the Boost Rtree.
	\item aMaxTree: The aggregate Max tree, built from the STX B+ tree, which stores an extra local range max value in each node. We use it for 1D MAX query comparison.
	\item Polyfit: Our proposed solution.
\end{enumerate}

\subsubsection{Deafult parameters}
Table \ref{tab:parameters} illustrates the involved parameters and their default values. Those default values are obtained through experimental tests.

\begin{table}[htbp]
	\centering
	\caption{Experimental Parameters}
	\label{tab:parameters}
	\begin{tabular}{|c|c|c|} \hline
		parameter & meaning & default \\ \hline
		$\epsilon$ & relative error threshold & 0.01 \\ \hline
		$\epsilon.abs$ & absolute error threshold & 100 \\ \hline
	\end{tabular}
\end{table}

\subsection{Hyperparameters Tuning}
\label{sec:hypertune}
In this section, we show how the relative error will affect the query response time and how to tune the most suitable absolute error threshold.

\subsubsection{Relative Error Threshold}

\begin{figure*}
	\centering
	\subfloat[Hit probability]{
		\includegraphics[scale=0.26]{figures/refinement.pdf}
	}
	\subfloat[Query response time when $\epsilon.abs=100$]{
		\includegraphics[scale=0.26]{figures/trelquerytime.pdf}
	}
	\subfloat[Query response time when $\epsilon.abs=50$]{
		\includegraphics[scale=0.26]{figures/trelquery50.pdf}
	}
	\caption{About relative error threshold}
	\label{fig:tuningTrel}
\end{figure*}

Figure \ref{fig:tuningTrel}(a) depicts the general relation between relative error threshold $\epsilon$ and the hit rate (i.e., the queries do not need refinement) under default absolute error setting (i.e., $\epsilon.abs=100$). It's clear that the tighter the relative error threshold is, the lower the hit probability and vise versa. Specifically, we maintain 96.3\% hit rate under the default setting ($\epsilon=0.01, \epsilon.abs=100$), which is good enough under most circumstances.

In Figure\ref{fig:tuningTrel}(b), we vary the relative error threshold $\epsilon$ to compare the average query response time with refinement under absolute error threshold 100. Where Polyfit-1, Polyfit-2 and Polyfit-3 denotes the Polyfit constructed using highest order 1, 2 and 3 respectively. Due to the number of models reduced, we can always faster than FITingTree by about 50ns. Though the number of models produced by Polyfit-1,2 and 3 are different, the query response time that caused mainly by tree traverse and model prediction do not differ a lot. As the tree height is log scale in terms of model amount. The advantage becomes more obvious when we come the the setting $\epsilon.abs=50$ (Figure \ref{fig:single_dimensional_aggregate}(c)), where we can be up to 2X faster than FITing-Tree.

\subsubsection{Aboslute Error Threshold}
\label{sec:optimalabs}

\begin{figure}[!hbt]
	\center
	\includegraphics[width=0.9\columnwidth]{figures/tabsquerytime.pdf}
	\caption{auto-tuning of absolute error}
	\label{fig:tabsquerytime}
\end{figure}

In Figure\ref{fig:tabsquerytime} we show how the absolute error threshold will affect the query response time with refinement under default relative error threshold (i.e., 0.01). Clearly, there exist an optimal $\epsilon.abs$ that produces the minimum average query response time (for a given relative error threshold), which balance the query time spent between model locating and query refinement. As shown in Figure \ref{fig:tabsquerytime}, the average query response time follow an "U" curve with its lowest point at around $\epsilon.abs=50$ to $\epsilon.abs=100$. Therefore, an exploratory search could be executed to find the optimal $\epsilon.abs$.


\subsection{The Performance of Polyfit}
\label{sec:performance}
In this subsection, we compare our proposed solution with all existing competitors on performance.

\subsubsection{Tuning the RMI method}
There is no instruction for how to choose the number of layers and models for the RMI structure, hence we need to tune the RMI to its best performance before comparison. This includes model selection, determination of layer amounts and the number of models in each layer. We use the TWEET dataset to tune the RMI, and the experiments including RMI will only be conducted on TWEET.

The first thing is model selection. In the experiment of \cite{kraska2018case}, they use a neural network with at most 2 hidden layer and 16 nodes in width for the top layer and linear regression for the leaf layer. In our experiment, we found that using a neural network is not appropriate for not only the leaf layer but also non-leaf layers. There are 2 reasons for this. First and also the most important, the time spent on neural network cloud be much longer compared with linear regression. Second, the accuracy of a shallow neural network is not remarkable compared with linear regression. Hence in the following experiments, all models of RMI are built with linear regression. As could be seen from table \ref{tab:model_comparison}, even using a neural network with only one hidden layer and 4 nodes will result in a prediction time more than 100ns on this single model.

\begin{table}[htbp]
	\centering
	\caption{Single RMI Model Comparison}
	\label{tab:model_comparison}
	\begin{tabular}{|c|c|c|c|c|c|c|} \hline
		Models & Architecture & Prediction time (ns) & Err.rel \\ \hline
		LR & / & 20 & 38.0\% \\ \hline
		NN & 1:4:1 & 119 & 24.1\% \\ \hline
		NN & 1:8:1 & 189 & 25.3\% \\ \hline
		NN & 1:16:1 & 275 & 25.3\% \\ \hline
		NN & 1:4:4:1 & 152 & 24.8\% \\ \hline
		NN & 1:8:8:1 & 347 & 21.4\% \\ \hline
		NN & 1:16:16:1 & 972 & 23.3\% \\ \hline
	\end{tabular}
\end{table}

Before tuning other hyperparameters of RMI, we temporarily remove the Btree replacement operation (and the error threshold) of RMI as it blocks us from measuring the relation between accuracy and the architecture. Now we explore the effect of choosing different number of models in both the bottom layer and the non-leaf layer. We notice that with the increasing of models in the bottom layer, the accuracy can drop quickly at the beginning. While when the accuracy goes to about 0.6\%, it becomes much harder to improve the accuracy by just increasing the number of models in the bottom layer. At this stage, increase the number of the non-leaf layer could help further improve the accuracy, but the improvement is very limited. Figure \ref{fig:tuningRMI}(a) gives the relation between the total number of models we used for the RMI and the accuracy it can achieve.

\begin{figure}
	\centering
	\subfloat[Accuracy and number of models]{
		\includegraphics[scale=0.19]{figures/compare_layer.pdf}
	}
	\subfloat[Query time and error threshold]{
		\includegraphics[scale=0.19]{figures/RMI_layer_time_replace.pdf}
	}
	\caption{tuning RMI}
	\label{fig:tuningRMI}
\end{figure}

When tuning the architecture, we fix the non-leaf layers with fanout 10 and vary the bottom layer model amount. Table \ref{tab:architecture} list the specific architecture we adopted for each point in figure \ref{fig:tuningRMI}(a). It's clear that under the same non-leaf architecture, more models in the leaf can always achieve better accuracy. It's also obvious that one can reorganize the models into a more layers architecture to achieve better accuracy while maintaining the total number of models unchanged.

\begin{table}[htbp]
	\centering
	\caption{RMI Architecture}
	\label{tab:architecture}
	\begin{tabular}{|c|c|c|c|c|} \hline
		\#Models & Architecture & Err.rel & Architecture & Err.rel \\ \hline
		101 & 1:10:90 & 2.90\% & / & / \\\hline
		201 & 1:10:190 & 1.63\% & / & / \\ \hline
		301 & 1:10:290 & 1.11\% & 1:10:100:190 & 0.91\% \\ \hline
		401 & 1:10:390 & 0.91\% & 1:10:100:290 & 0.63\% \\ \hline
		501 & 1:10:490 & 0.69\% & 1:10:100:390 & 0.49\% \\ \hline
		1001 & 1:10:990 & 0.37\% & 1:10:100:890 & 0.27\% \\ \hline
		1501 & 1:10:1490 & 0.23\% & 1:10:100:1390 & 0.17\% \\ \hline
	\end{tabular}
\end{table}

When we ignore the Btree replacement operation, the query response time of RMI is much easier to explain as it is simply linear to the number of layers of the stage model. However, when we consider the Btree replacement operation, the query response time becomes highly unstable/unpredictable. As one cannot know whether one query will be distributed to a bottom layer model that has been replaced by a Btree and how height the Btree is. The query response time with regard to the error threshold is given in figure \ref{fig:tuningRMI}(b). The 4 layer RMI with architecture 1:10:100:1000 can achieve the least query response time among wide range mainly because the accuracy contributed by its architecture results is less bottom model be replaced by Btree and hence a lot Btree traverse time could be saved. The 2 layer RMI with architecture 1:1000 could perform better than the 3 layer RMI with architecture 1:10:1000 and some times even better than the 4 layer RMI. This because when the error threshold is large enough, very few bottom models are replaced with Btree and the advantage of fewer layers can save more query response time. Similarly, when the error threshold is small enough, nearly all bottom model is replaced with Btree, and once again the less layer advantage starts to show. In the following comparison, we choose the best architecture of RMI we can find under each comparison condition.	

\subsubsection{1D Count Queries}

We first compare our method with the error guaranteed sampling (i.e., S2) only as it's the only one in our competitors that could guarantee relative error without any modification.
Table \ref{tab:comparewiths2} gives the comparison result under default setting. Specifically, we set the probability threshold of S2 to 90\%, which is slightly lower than the measured hit rate of our method. The performance of S2, however, is much slower than our method, as the tight relative error threshold and probability requirement make S2 perform a lot of sampling until the termination condition is satisfied.

\begin{table}[htbp]
	\centering
	\caption{Compared With S2}
	\label{tab:comparewiths2}
	\begin{tabular}{|c|c|c|c|c|} \hline
		Method & Query Time (ns) & $\epsilon$ & Probability & Hit rate \\ \hline
		Polyfit-2 & 99 & 0.01 & / & 96.3\% \\ \hline
		S2 & 35,628,445 & 0.01 & 90\% & / \\ \hline
	\end{tabular}
\end{table}

\begin{figure*}
	\centering
	\subfloat[compared with traditional methods]{
		\includegraphics[scale=0.27]{figures/accuracy_querytime_ROL_hist_stx.pdf}
	}
	\subfloat[compared with FITing-Tree]{
		\includegraphics[scale=0.27]{figures/accuracy_querytime_ROL_atree.pdf}
	}
	\subfloat[compared with RMI]{
		\includegraphics[scale=0.27]{figures/accuracy_querytime_ROL_RMI.pdf}
	}
	\caption{Query time with regard to accuracy}
	\label{fig:comparison_accuracy_querytime}
\end{figure*}

Then, we compare the query time and accuracy trade-off. Since the methods for comparison have their own hyper-parameters, we no longer vary the absolute error threshold or the relative error threshold directly in this section. Instead, we measure the real relative error and the corresponding average query response time without refinement. Such that we can compare them in a unified form. In addition, we also divide the comparison result into three parts, due to the vast difference of their performance.

As shown in figure \ref{fig:comparison_accuracy_querytime}(a), Polyfit can keep the best performance while the histogram method is the worst. Sampling combined with Btree (i.e., STX) can achieve similar performance when the required accuracy is low. When the required accuracy goes higher (i.e., the relative error goes smaller), the query response time of STX method raise dramatically, this mainly due to the increase of layers in the Btree. Figure \ref{fig:comparison_accuracy_querytime}(b) compare our method with FITing-Tree. Obviously, our method outperforms FITing-Tree over the entire accuracy domain. With the increasing of accuracy, the advantage of our method becomes more prominent.

Figure \ref{fig:comparison_accuracy_querytime}(c) compare our method with RMI. RMI is quite interesting, as the performance is affected by both their architecture and the error threshold. We hence implement 3 versions of the RMI to cover the accuracy domain. As shown, RMI-1000 has the bottom layer model amount to be 1000, RMI-500 has the bottom layer model amount to be 500 and RMI-100 has the bottom layer model amount to be 100. We vary the number of layers of each RMI method to obtain the best query response time under the same error threshold. We then vary the error threshold to obtain the change between accuracy and best query response time. It's clear that Polyfit can outperform RMI over various of settings. But in some case, RMI is able to achieve better performance under well-tuned architecture and relaxed error threshold (i.e., no model is replaced by Btree in such error threshold) such that no time is spent on traversing the Btree. While Polyfit is much more stable over the accuracy domain. It's mainly contributed from the much fewer models we used to approximate the dataset.

\subsubsection{1D MIN/MAX Queries}
For min/max query. We use a financial dataset that records the Hong Kong 40 Index of 2018 \cite{hk40index}, which contains about 0.9M records. The query set is generated with Gaussian distribution with sigma 10000. We list the comparison with an aggregate max tree that produces exact result in table \ref{tab:max_comparison}, which gives the average query response time. Specifically, when $\epsilon.abs=100$, we are 2.5X faster.

\begin{table}[htbp]
	\centering
	\caption{Max Query Comparison}
	\label{tab:max_comparison}
	\begin{tabular}{|c|c|c|} \hline
		$\backslash$ & Polyfit & aMaxTree  \\ \hline
		query time & 1357 ns& 3289 ns \\ \hline
	\end{tabular}
\end{table}

\subsubsection{2D Performance}

\begin{figure}[!hbt]
	\centering
	\subfloat[Response time]{
		\includegraphics[scale=0.20]{figures/2D_comparison.pdf}
	}
	\subfloat[2D queries]{
		%\includegraphics[scale=0.26]{figures/2D_queries.pdf}
	}
	\caption{the 2-dimensional query response time and its corresponding queries}
	\label{fig:2D_comparison}
\end{figure}

For 2D count query, we use 100 million records from \cite{osmplanet2019} as the dataset and generate the corresponding cumulative COUNT surface. Our models are trained to approximate this surface within absolute error threshold 1000. We compare the 2-dimensional COUNT query response time with an aggregate Rtree. The query set contains 300 queries generated by Gaussian distribution where the sigma is set to be 10\% of the corresponding domain size.

As shown in figure \ref{fig:2D_comparison}, our method achieve relative stable query response time with different relative error threshold $\epsilon$. Though aggregate Rtree produces exact result, it's 13X slower even under 0.1\% relative error threshold.

\subsection{Why OptSeg is Necessary}
\label{sec:whyoptseg}

\begin{figure*}
	\centering
	 \subfloat[Absolute error and number of models]{
		\includegraphics[scale=0.26]{figures/modelamount.pdf}
	}
	\subfloat[Query response time when $\epsilon.abs=100$]{
		\includegraphics[scale=0.26]{figures/abserr_segments.pdf}
	}
	\subfloat[Query response time when $\epsilon.abs=50$]{
		\includegraphics[scale=0.26]{figures/bins_querytime.pdf}
	}
	\caption{About segmentation on TWEET}
	\label{fig:segmentation_exp}
\end{figure*}

% model amount (Fiting tree, Polyfit 1 2 3) - T.abs
We first demonstrate the advantage of our segmentation algorithm (and curve fitting) by evaluating the number of models generated under the same absolute error threshold $\epsilon.abs$. Figure \ref{fig:segmentation_exp}(a) shows the results of this experiment. It's obvious that our techniques produce the least number of models under the same error threshold. This mainly due to the optimization step that fully utilizes the absolute error threshold budget. Such that we always produce the least number of model to cover a dataset. Specifically, when $d=3$, we use only 34.8\% of the models needed for FITingTree. Notice in this comparison, we also include the well known Douglasa Peucker ($Dogulas$) algorithm, which served as a reference here.

We then show the necessity of the segmentation algorithm by replacing OptSeg with the segmentation produced by Entropy Histogram \cite{to2013entropy} (i.e, the Hist method). As denoted in Figure \ref{fig:segmentation_exp}(b)'s EntropyHist, we first use Entropy Histogram to generate the segmentation, then we use Polyfit to fit each segment. Such that the only difference now is only segmentation algorithm. After that, the COUNT query's error is measured to generate the measured absolute error - segmentation curve. In comparison, we also plot the absoluter error threshold - number of segmentation curves of our method (i.e., Polyfit-1,2,3, that also appear in (a)). Finally, we vary the number of bins for the above mentioned Entropy Histogram segmentation replacement method and tune it to its optimal. We can see from \ref{fig:segmentation_exp}(c) that even in its best performance, it's slower than our method under the default parameter settings.

\subsection{Other Features}
\label{sec:otherfeatures}
\begin{figure*}
	\centering
	\subfloat[Scale on OSM]{
		\includegraphics[scale=0.26]{figures/dataset_querytime.pdf}
	}
	 \subfloat[Construction time]{
		\includegraphics[scale=0.26]{figures/constructiontime.pdf}
	}
	\subfloat[Accuracy and number of parameters]{
		\includegraphics[scale=0.26]{figures/parameter_accuracy_all.pdf}
	}
	\caption{Polyfit features}
	\label{fig:GIS features}
\end{figure*}

\subsubsection{Robustness to Scale}
We evaluate the robustness of our algorithm in terms of data scale on OSM dataset. Where we vary the dataset size from 1M to 100M. As shown in Figure \ref{fig:GIS features}(a), we achieve stable performance and are faster than FITing-Tree with more significant advantage on greater dataset size.

\subsubsection{Construction Time}
The construction time figure (Figure \ref{fig:GIS features}(b)) also follow common sense. The higher the absolute error is, the higher the construction time will be. As higher absolute error will allow more data records fit in 1 model, which increase the number of condition in linear programming. And hence the construction time. Luckily, we could enable finer granularity more easily with this feature.

\subsubsection{Accuracy vs Size}
Figure \ref{fig:GIS features}(c) shows the relationship between each method's size and its accuracy. The RMI is able to outperform traditional scan-based methods (i.e., histogram and sampling with Btree) by using the same space to achieve higher accuracy (i.e., lower relative error). The FITing-Tree method can further improve the accuracy a little. While Polyfit can achieve the highest accuracy with the same space limit. This improvement all comes from the max loss model, the adaptive step and regression correction techniques that reduce the number of models required to approximate the data distribution under the same error threshold. In conclusion, compared with FITing-Tree and RMI, we can reduce the size by up to 40\% and 50\% respectively under the same accuracy. Notice when calculating the size, we use the minimum amount of parameter for each method, such that a linear regression use only two parameters (or three if the model has a fixed domain), a b+ tree takes only all the keys and pointers. 

==> old_case_2d.tex <==
\section{Approximate Range Aggregate Queries with two keys}
\label{sec:extend_2d}
In previous sections, we mainly focus on range aggregate queries, in which each element only contains one single key (cf. Definition \ref{def:RAQ}). However, existing work \cite{heimel2015self,riondato2011vc,gunopulos2005selectivity,gunopulos2000approximating} also support range aggregate queries with two keys for each element. In this section, we discuss how to extend our techniques in this setting (cf. Definition \ref{def:2D_Approx_RAQ}). As a remark, our techniques can be also extended to the setting of multiple keys. Here, we only focus on count query. However, we can also adopt our methods for other types of range aggregate queries.

\begin{definition}
\label{def:2D_Approx_RAQ}
Given $\mathcal{D}$ as a set of elements $(u, v, w)$, where $u$, $v$ and $w$ are the first key, second key and the weight respectively, and the ranges of keys are $[L_1, U_1]$ for $u$ and $[L_2, U_2]$ for $v$, we define $\mathcal{D}[L_1,U_1][L_2,U_2]$ as the subset of $\mathcal{D}$ such that all the keys $(u,v)$ are within the above region, i.e.,
\begin{equation*}
\mathcal{D}[L_1,U_1][L_2,U_2]=\sigma_{u\in [L_1,U_1], v\in [L_2,U_2]} (\mathcal{D})
\end{equation*}
The count query is defined as:
\begin{equation}
\label{eq:2D_count}
R_c(\mathcal{D}[L_1,U_1][L_2,U_2])=|\mathcal{D}[L_1,U_1][L_2,U_2]|
\end{equation}
\end{definition}

Instead of building the key-cumulative array (cf. Figure \ref{fig:key_cumulative_array}) for solving the count query, we build the following key-cumulative function to represent the surface (cf. Figure \ref{fig:example2D}), which are formally stated in Definition \ref{def:accu2D}.
%

%\begin{figure}[!hbt]
%%\vspace{-8mm}
%\centering
%\subfloat[Data]{\includegraphics[scale=0.30]{figures/2D_dataset.pdf}}
%\subfloat[Key cumulative function]{\includegraphics[scale=0.30]{figures/2D_accumulation.png}}
%%\vspace{-3mm}
%\caption{Tweet dataset \cite{chen2015temporal} with longitude and latitude as the keys}
%%\vspace{-3mm}
%\label{fig:example2D}
%\end{figure}

\begin{figure*}[!hbt]
\center
\subfloat[tweet locations as data points]{ \includegraphics[width=0.65\columnwidth]{figures/discrete_2D.pdf} }
\subfloat[function for range SUM queries]{ \includegraphics[width=0.7\columnwidth]{figures/continue_2D_sampled.pdf} }
%\includegraphics[width=0.9\columnwidth]{figures/fx_LS_LR_data_sampled_1_100.pdf}
\caption{Tweet locations, 2-dimensional keys: discrete data points vs. continuous function}
\label{fig:example2D}
\end{figure*}



\begin{definition}
%\vspace{-2mm}
\label{def:accu2D}
The key-cumulative function with two keys for count query is defined as $CF_{G_c}(u,v)$, where:
\begin{eqnarray}
\label{eq:accu2d}
CF_{R_c}(u,v) = R_c(\mathcal{D}[-\infty, u][-\infty, v])
\end{eqnarray}
\end{definition}

Therefore, we can solve the count query $R_c(\mathcal{D}[L_1,U_1][L_2,U_2])$, using the following equation.
\begin{equation*}
\begin{split}
R_c(\mathcal{D}[L_1,U_1][L_2,U_2])=CF_{R_c}(L_2,U_2)-CF_{R_c}(L_2,U_1)\\
-CF_{R_c}(L_1,U_2)+CF_{R_c}(L_1,U_1)
\end{split}
\end{equation*}

Then, we follow the similar idea in Section \ref{sec:min_error} and utilize the polynomial surface $\mathbb{P}(u,v)$ to approximate the key cumulative function $CF_{R_c}(u,v)$ with two keys, where:
$$\mathbb{P}(u,v)=\sum_{i=1,i+j\leq d}^d a_{ij} u^i v^j$$

By replacing $F(k_i)$ and $\mathbb{P}(k_i)$ in Equation \ref{eq:error} by $F(u_i,v_i)$ and $\mathbb{P}(u_i,v_i)$ respectively, we can obtain the similar linear programming problem for obtaining the best parameters $a_{ij}$. However, unlike the one-dimensional case, it takes at least $O(n^2)$ to obtain the minimum number of segmentations by using the GS method (cf. Section \ref{sec:GS}), which is infeasible even for small-scale dataset (e.g., 10000 points). As such, we propose to utilize the Quad-tree based solution to obtain the segmentation. \edison{add figure to illustrate this concept.} 
